Nukhada USV: a Robot for Autonomous Surveying and Support to Underwater Operations

The Technology Innovation Institute in Abu Dhabi, United Arab Emirates, has recently finished the production and testing of a new unmanned surface vehicle, called Nukhada, specifically designed for autonomous survey, inspection, and support to underwater operations. This manuscript describes the main characteristics of the Nukhada USV, as well as some of the trials conducted during the development.

==> Sections/abstract_submission.tex <==
% MOTIVATION
As the era of space exploration is taking off, we still know very little about our oceans. It is estimated that more than 80\% of the marine environment remains unexplored. Yet, the few we know about, serves a key role in our economic infrastructure, as the oceans provide a great source for energy production and natural resources extraction, as well as transport media. Unravelling the mysteries of such an environment, as well as preserving it for a sustainable future, is becoming an increasingly attractive challenge for the scientific community.

% BACKGROUND / RELEVANCY
The Technology Innovation Institute (TII) of Abu Dhabi, United Arab Emirates, started in 2020 an ambitious project towards the understanding and preservation of our oceans. In this context, we are developing marine robotic platforms that can support us on our project on cooperative exploration missions, human-made structure inspection and maintenance, and among many others, search and rescue. This paper presents the first \ac{USV} robot of our fleet of marine vehicles, the Nukhada~USV (see \fref{fig:nukhada}), and its scaled version for easy prototyping, the Nukhada-mini~USV (see \fref{fig:nukhada_mini}). In particular, we focus on the mechanical design and software architecture of the vehicles, whose construction and initial testing finished in July 2021, and we are working to get them fully operative by the end of 2021. We believe that this paper, as previous publications of similar nature, e.g.,~\cite{ribas2011girona,carreras2015testing,willners2021from}, is of relevance to the robotics community as it can serve as inspiration to the community at large for the hardware and software design of future marine platforms.

% PHYSICAL CONSTITUTION (one paragraph)
The catamarans Nukhada~USV and its scaled version have symmetric double-ender hulls. The spacing between the demi-hulls is strategic for the support of \acp{AUV} in underwater robotic operations, as it allows for their docking and charging. Approximately, the size of the Nukhada~USV is ${6 \times 3.5}$~metres, whereas the scaled version is ${1.2 \times 0.45}$~metres. The full-scaled USV is constructed in a modular way to allow for easy transportation. Its propulsion system consists of two independently steerable electric pod engines and four rudders. This setup enables high manoeuvrability in confined spaces, as well as a 6~kn and 10~kn of cruise and maximum speed, respectively. The vehicle is powered up with a set of LiFePo4 batteries totalling 10.56~kWh, providing an approximate autonomy of 100~NM.

% PAYLOAD and HARDWARE DESCRIPTION (one paragraph)
The vehicle is equipped with a range of varied sensing that ensures essential health monitoring (e.g., \ac{BMS} and water sensors), communications (e.g., \ac{USBL}) and localisation (e.g., \ac{IMU} and \ac{DVL}). Additionally, a platform connecting both hulls serves as a multi-purpose dry payload area with a capacity of 600~kg for a range of additional sensors (e.g., \ac{AIS}, \ac{GNSS}, radar, cameras and \ac{LiDAR}), as well as for landing area of \acp{UAV}. A wet payload area below the waterline allows for the integration of underwater sensing (e.g., \ac{FLS}, cameras and echosounders).

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.9\columnwidth]{./Figures/nukhada.jpg}
    \caption{Nukhada~USV, TII's new USV for autonomous survey, inspection, and support to underwater robotic operations.}
    \label{fig:nukhada}
\end{figure}

\begin{figure}[b!]
    \centering
    \includegraphics[width=0.7\columnwidth]{./Figures/nukhada_mini.jpg}
    \caption{Nukhada-mini~USV, a scaled version for steadily and safely progress from algorithmic prototyping to application deployment in real-world challenging scenarios.}
    \label{fig:nukhada_mini}
\end{figure}

% SOFTWARE DESCRIPTION (one paragraph)
The Nukhada~USV autonomy architecture consists of three main functional modules (see \fref{fig:nukhada_architecture}). Firstly, the \textit{frontseat} interfaces the essential actuators and various interoceptive and exteroceptive sensors to endow the robot with fundamental safety, communication, localisation and control routines. To the interest of this paper, we highlight the cascaded low-level controller strategy that allows guiding the vehicle towards position, velocity and force setpoints. Secondly, the \textit{backseat} extends the vehicle's capabilities with more sophisticated algorithms for docking, mapping, and among others, path planning and tracking. Finally, the \textit{payload} includes some additional exteroceptive sensors to feed the whole robot autonomy architecture with richer information about the surrounding environment. All these functional blocks run on Linux Ubuntu powered by the \ac{ROS}~\cite{quigley2009ros}.

% FULL vs SCALED (one paragraph)
A peculiarity of our Nukhada~USV is the parallel development of its scaled version, the Nukhuda-mini USV. The scaled vehicle is equipped either with the same or cheaper hardware alternatives (but with the same sensor technology) than the full-scale USV, while their software architecture is the same. That allows us to include an intermediate step between simulations and real-world deployment, consisting of small-scale testing in controlled spaces, while preventing the need to heavily modify sensor-fusion and control strategies when migrating algorithms between vehicles. Given the size of our Nukhada~USV, having an easier to deploy, scaled version is particularly relevant as most controlled spaces are water or waves tanks of reduced space, and testing in open waters with the final platform requires more attention to safety.

\begin{figure}[t!]
    \centering
    \includegraphics[width=\columnwidth]{./Figures/nukhada_architecture.jpg}
    \caption{Nukhada's autonomy architecture.}
    \label{fig:nukhada_architecture}
\end{figure}

% CONTENT OF THE FINAL PAPER
In the final paper, we will provide a detailed description of the design aspects and constituent hardware of our Nukhada~USV. We will also discuss the software architecture that powers the autonomy of our vehicles. Finally, we will elaborate on our vision of using the scaled version of the USV to steadily and safely progress from algorithmic prototyping to application deployment in real-world challenging scenarios.

==> Sections/mechanical_design_spin.tex <==
Approximately, the size of the Nukhada~USV is ${6 \times 3.5}$~metres, whereas the scaled version is ${1.2 \times 0.45}$~metres.6~kn and 7~kn of cruise and maximum speed, respectively.

Simone Spanò – Mechanical Design main charactheristics
The catamarans Nukhada~USV is a light modular autonomous surface vessel for the deployment of underwater ROVs.
The catamarans Nukhada~USV has symmetric double-ender hulls. The spacing between the demi-hulls is strategic for the support of \acp{AUV} in underwater robotic operations, as it allows for their docking and charging.


Modularity
•	Each hull made of three 2m-long watertight sections joint together.
•	Design allows scope to re-use hull sections in different hull configurations (longer…larger).
•	Swappable hull sections guarantee ease of maintenance and low downtime.
•	Fast and secure coupling techniques between hulls.
•	The platform between the two hulls is also modular; you can vary the width, length, height and arrangement of the various sections of the platform.

Versatility
•	Hybrid propulsion guarantees large operational range.
•	Electric engines allow for virtually silent and environmentally friendly operations.
•	Hull sections can be pre-configured and fitted according to different mission requirements.
•	presence of rails on both sides of each section to allow for quick assembly of additional components.

Ease of transport, assembly and deployment
•	Hull and upper platform sections are no longer than 2m.
•	The whole vessel can be conveniently stored and shipped in pieces
•	Assembly of the vessel requiring basic tools (screwdriver, wrenches, pliers) and no glue/adhesive
•	Narrowing of the width of the catamaran to allow the transport on road by trailer.
•	presence of hooking points for the trailer by means of ropes, placed either on the stern and the bow. 
•	presence of hooking points for lifting, placed in correspondence of the interface plates of each section of the catamaran.

Robust marine design
•	Proven seakeeping qualities.
•	Two steerable independent pod engines and optionally, four rudders guarantee unmatched manoeuvrability in confined spaces.
•	Redundancy in case of failure: Each central Hull section is independent. The catamaran can be manoeuvred only with one motor and one rudder.	
•	Large flat surfaces available for safe transport of mission payload, or Solar panel installation.

Sensors/ control
•	Radar/Lidar/GPS RTK/IMU/USBL Master/Camera.
•	Remote control / Path tracking / obstacle avoidance / auto docking.

==> Sections/power_system_and_computer_architecture.tex <==
Simone Spanò – Power system and connected devices
The USV catamaran is powered by batteries and is equipped with a diesel-electric generation system to extend its range. Both the batteries and the diesel generator are located inside the two central hulls.
The devices requiring power located inside the catamaran are positioned both inside the central hulls and outside the hulls, i.e. on the platforms that can be used to add payloads.
Inside each of the two central hulls there is: 
•	Diesel range extender providing 2.5KW designed to recharge the batteries.
•	Battery Management System designed to monitor 16 cells in series battery pack. All he typical parameters monitored by BMS are sent via CAN BUS.
•	Battery pack consisting of 16 LiFePO lithium cells (3.2V / 110Ah) in series, providing 5.6KWh at 52VDC. The battery pack can be doubled to increase the autonomy of the catamatan. Each catamaran has the battery packs of one hull and the other connected in parallel in order to have a balanced charge of the two different battery packs.
•	Pod rotation controller, pod rotation hollow shaft gearbox and pod rotation motor, which allow the engine pod to be rotated by +/-180° both with the catamaran stationary and in motion.
•	Pod engine controller and pod engine. The pod engine is an in-water motor in a watertight aluminium casing. Equipped with a through-hull tube for mounting through the hull. The motor controller is powered at 48VDC and the Pod engine provides maximum 4.3KW on the shaft at 1350rpm.

The catamaran with the standard equipment has an estimated range at cruise speed of 4 Knots of 20 Nautical miles. The maximum speed is 8 Knots

Outside the hull, attached to the central platform that connects the two hulls, there are two compartments: the "Junction Box" and the "USV control box", which contain various devices used for the autonomous driving of the catamaran.
In the junction box there is:
•	A switch (on/off switch) to turn on the POD Engine controller.
•	An electronic board (USV speed and direction controller), connected via CAN Bus with the "USV Computer" with the function of sending information to the POD engine controller regarding the speed of rotation of the PODs and the direction of rotation of the PODs.
•	Two displays indicating the status of the two POD controllers.
•	Two DC/DC converters with 48VDC input, one with 24VDC output (powering the "USV speed and direction controller" and the "modem router wi-fi/4G") and one with 12VDC output (powering the "USV computer and display" and the "LIDAR computer").

In the USV control box there is:
•	"USV computer and display" which is the main computer that performs the functions of path planner, path follower, obstacle avoidance and sensor reading. This computer is connected via Ethernet to the modem. The USB/CAN converter is connected to this computer.
•	"LIDAR computer" which has the function of receiving the point cloud from the LIDAR sensor and returning obstacle detection information. This is connected via Ethernet to the Router.
•	"Modem Router wi-fi / 4G" which has the function of routing data packets between the various devices and communicating with them via wi-fi and 4G

